General Knapsack Problems in a Dynamic Setting

The world is dynamic and changes over time, thus any optimization problem used to model real life problems must address this dynamic nature, taking into account the cost of changes to a solution over time. The multistage model was introduced with this goal in mind. In this model we are given a series of instances of an optimization problem, corresponding to different times, and a solution is provided for each instance. The strive for obtaining near-optimal solutions for each instance on one hand, while maintaining similar solutions for consecutive time units on the other hand, is quantified and integrated into the objective function. In this paper we consider the Generalized Multistage $d$-Knapsack problem, a generalization of the multistage variants of the Multiple Knapsack problem, as well as the $d$-Dimensional Knapsack problem. We present a PTAS for Generalized Multistage $d$-Knapsack.

==> discussion.tex <==
In this paper we considered the Generalized Multistage $d$-Knapsack problem. A PTAS was presented for the modular variant, while a $\left(1-\frac{1}{e}\right)$-approximation algorithm was presented for the monotone submodular variant. Both algorithms use the same framework, split the time horizon into sub instance, and solve each sub intsance by reducing it to the $d$-MKCP problem for which an algorithm exists.

Any instance of $d$-GMK includes either submodular profit functions or change costs.
Including both traits is not supported by our algorithm due to limitations of the algorithm for $d$-MKCP \cite{fairstein2020tight}, derived from continuous submodular optimization algorithms \cite{calinescu2007maximizing,feldman2011unified}. These algorithm are restricted to the optimization of non-negative functions. Since the value of an element in our reduction may decrease and become negative, we cannot guarantee this in general instances.

In this paper we considered modular and monotone submodular profit functions. A natural generalization would be to consider non-monotone submodular profit functions. The algorithm presented in this paper does not handle non-monotone submodular functions, even though the approximation algorithm for $d$-MKCP \cite{fairstein2020tight} supports non-monotone functions. This is due to the reduction used, which does not preserve submodularity of non-monotone functions and results in an objective function that is not submodular.


